Efficient Medical Image Assessment via Self-supervised Learning

High-performance deep learning methods typically rely on large annotated training datasets, which are difficult to obtain in many clinical applications due to the high cost of medical image labeling. Existing data assessment methods commonly require knowing the labels in advance, which are not feasible to achieve our goal of 'knowing which data to label.' To this end, we formulate and propose a novel and efficient data assessment strategy, EXponentiAl Marginal sINgular valuE (EXAMINE) score, to rank the quality of unlabeled medical image data based on their useful latent representations extracted via Self-supervised Learning (SSL) networks. Motivated by theoretical implication of SSL embedding space, we leverage a Masked Autoencoder for feature extraction. Furthermore, we evaluate data quality based on the marginal change of the largest singular value after excluding the data point in the dataset. We conduct extensive experiments on a pathology dataset. Our results indicate the effectiveness and efficiency of our proposed methods for selecting the most valuable data to label.

==> 02-problem.tex <==
\section{Preliminary}
\subsection{Data valuation problem setting}
\Li{1. Please refer to Zou's and Liang's paper and write down the problem setup, including goal, assumption, input, output, and corresponding math formulation.\\
2. Please write down the weakness of the existing data valuation methods (e.g. requiring supervised training, time costly, etc.)}
\subsection{Self-supervised learning-based feature embedding }
\Li{General description without math}



==> 07-proof.tex <==
\section{Appendix}

\subsection{Dataset Details}
\label{app_data}


\todo{A table of the dataset}
\todo{A table of hyper-parameters}


\subsection{Additional ablation studies}


\subsection{Detailed model architectures}


\begin{table*}[h]
\centering
\begin{tabular}{c|c}
\toprule
\textbf{Layer}              & \textbf{Details}    \\ \midrule  
1   & Dropout($p$ = 0.1)  \\ \hline
2 & G-conv($D$, 256) + ELU                     \\ \hline
3 & G-conv(256, 64) + ELU                     \\ \hline
4 &  FC(64, 1)  +Sigmoid                     \\ \hline
5  & Random-vector(4)  \\ \hline
6 & Linear(68, 128) + ReLU+BN(128)                   \\ \hline
7 & Linear(128, 256)  + ReLU+BN(256)                   \\ \hline
8 & FC(256, $D$) +   tanh                  \\ \hline
9 & Linear($D$, 32)  ReLU                   \\ \hline     
10 & FC(32, 2)                 \\ \bottomrule  
\end{tabular}
\caption{ Network architecture of the missing node generator.}
\label{tab_arch1}
\end{table*}


